BROOD: Bilevel and Robust Optimization and Outlier Detection for Efficient Tuning of High-Energy Physics Event Generators

The parameters in Monte Carlo (MC) event generators are tuned on experimental measurements by evaluating the goodness of fit between the data and the MC predictions. The relative importance of each measurement is adjusted manually in an often time-consuming, iterative process to meet different experimental needs. In this work, we introduce several optimization formulations and algorithms with new decision criteria for streamlining and automating this process. These algorithms are designed for two formulations: bilevel optimization and robust optimization. Both formulations are applied to the datasets used in the ATLAS A14 tune and to the dedicated hadronization datasets generated by the sherpa generator, respectively. The corresponding tuned generator parameters are compared using three metrics. We compare the quality of our automatic tunes to the published ATLAS A14 tune. Moreover, we analyze the impact of a pre-processing step that excludes data that cannot be described by the physics models used in the MC event generators.

==> Makefile <==
TEXROOT=DOE_main_SciPost
TEXFILES= DOE_main_SciPost.tex app_conclusion.tex app_intro.tex app_metric.tex app_numerical.tex app_optimization.tex \
	app_problem.tex bilevel.tex conclusion.tex discussion.tex eigen.tex \
	hypofilter.tex introduction.tex macros.tex obsfilter.tex results.tex robopt.tex svensway.tex
SuppTEXFILES= 
PICS=
EPSS=
BIBFILES= biblio.bib MPEC.bib

all: $(TEXROOT).pdf

# latex & bibtex main file
$(TEXROOT).pdf: $(TEXFILES) $(PICS) $(BIBFILES)
	pdflatex $(TEXROOT).tex \
	bibtex $(TEXROOT) \
	pdflatex $(TEXROOT).tex \
	bibtex $(TEXROOT) \
	pdflatex $(TEXROOT).tex \

# create pictures, if needed
.SUFFIXES: .fig .pdf

#.fig.pdf:
#	fig2dev -L pdf $< $@

clean:
	rm -f $(TEXROOT).pdf *.aux *.bbl *.blg *.toc *.log *.bak *.out *.thm *synctex.gz *~

reallyclean: clean
	rm -f pics/*.pdf


